The BitTorrent Anonymity Marketplace

The very nature of operations in peer-to-peer systems such as BitTorrent exposes information about participants to their peers. Nodes desiring anonymity, therefore, often chose to route their peer-to-peer traffic through anonymity relays, such as Tor. Unfortunately, these relays have little incentive for contribution and struggle to scale with the high loads that P2P traffic foists upon them. We propose a novel modification for BitTorrent that we call the BitTorrent Anonymity Marketplace. Peers in our system trade in k swarms obscuring the actual intent of the participants. But because peers can cross-trade torrents, the k-1 cover traffic can actually serve a useful purpose. This creates a system wherein a neighbor cannot determine if a node actually wants a given torrent, or if it is only using it as leverage to get the one it really wants. In this paper, we present our design, explore its operation in simulation, and analyze its effectiveness. We demonstrate that the upload and download characteristics of cover traffic and desired torrents are statistically difficult to distinguish.

==> evaluation.tex <==
We have established three hypotheses we wish to evaluate in this paper. We have evaluated our proposed BitTorrent Anonymity Marketplace for
each of these hypotheses. These three hypotheses reduce to evaluating the Marketplace in terms of:

\begin{enumerate}
\item Anonymity
\item Download Costs
\item Incentives
\end{enumerate}

We evaluated the first two of these using simulation, and the second in a more % XXX second --> third?
qualitative fashion. For simulation, we extended an event driven BitTorrent simulator
that we developed In previous research~\cite{longterm}.

We could have also evaluated our work using true clients on an artificial network such as
Plaentlab. However, we saw minimal advantages to such an evaluation and many advantages
to using pure simulation. The largest advantage was the ability to run simulations many times
faster than real-time. This was especially appropriate given the need to tweak small
parameters to the aforementioned torrent evaluation function and then re-test. Alternatively,
% XXX: insert a (see Section~\ref{...}) for the "aforementioned" function
we could have released a Marketplace client for general evaluation, but given the lack of
backwards compatibility and potential legal issues, we decided that simulation was a better first step.

The simulation tested for our research was parameterized as follows:

\begin{itemize}
\item $k$ = 5
\item 100 peers
\item 40 torrents
\item 125MB sized files
\item Peer upload/download 1Mbps
\end{itemize}

The simulation ends when all clients have downloaded their native interest
and at least $k-1$ additional torrents. The simulation was executed twenty times.
% XXX say something about memory use, simulation runtimes, etc.  Impress us with how
% long these things take to run and how many different simulations you ultimately ran.
% Make it clear that, despite the seemingly ad-hoc nature of the design of these things,
% we exhaustively simulated the parameter space that we set up, and found some interesting results.

\subsection{Anonymity Evaluation}

The primary goal of the BitTorrent Anonymity Marketplace is indistinguishability of intent.
That is, a node downloading $1$ native interest, and $k-1$ non-native interests will not
reveal which of the $k$ torrents is the native interest. In particular, the node's peers
cannot determine, with a high degree of certainty,  the node's native interest from their protocol interactions.

To quantify ``high degree of certainty'' our primary evaluation metric graphs the behavior of nodes with respect
to their native downloads and non-native downloads. The graphs show averages and standard deviations. 
We accept results where the average behavior of the native group is within the 
standard deviation of the behavior of the non-native group.

\paragraph{Start Time.} We first evaluate the indistinguishability of start times, where start time is
measured as an integer rank. In other words, the first torrent that a node makes requests for is ranked $1$, 
and the second torrent that a node makes requests for is ranked $2$, and so on. We evaluated this
aspect of indistinguishability in two ways.

First, we checked that there was sufficient variability of start times for native interests. It is important, of course,
that native interests not have a predictable start rank. Our results are shown in Figure~\ref{native_startrank}. 
The graph is parameterized on the number of nodes natively interested in the node, as a measure of popularity.
The y axis is the average start rank for nodes of that popularity and the standard deviation. The graph shows
that the standard deviation is high for start rank, so a node's native interests are suitably obscured from its peers.

\begin{figure}
\centering
\includegraphics[scale=.25]{native_startranks.png}
\caption{The mean start rank of native interests plotted against popularity. 
The X axis is the number of peers natively interested in the torrent, the Y
axis is the starting rank. The error bars show the standard deviation. The 
wide standard deviations means that native interests have a wide
range of start rank.\label{native_startrank}}
\end{figure}

Our second measure of the indistinguishability of start times is to measure the
average start time for the same torrent for peers that are natively interested relative to
peers that are not (see Figure~\ref{startranks_cmp}). % As shown by this figure,
There is a noticeable shift to earlier start times for native interests. Nevertheless, 
the average times for the native interests lie within the standard deviations of the
start times for non-native interests. Perhaps more importantly, the native and non-native
graphs have similar shapes, suggesting similar behavior for the two populations.

\begin{figure}
\centering
\includegraphics[scale=.25]{native_nonnative_startranks.png}
\caption{The mean start rank of the various torrents plotted against 
the start rank for the same torrent for peers not natively interested. This graph shows
that native interests do start sooner, but the mean lies within the standard deviation 
of non-native interest start times for most torrents.\label{startranks_cmp}}
\end{figure}

\paragraph{End Time.} It is also important that native interests not end at a predictable time.
Again, expressing end times as integer ranks, we evaluate the variability of native start times in Figure~\ref{native_endrank}
and compare those times to non-native end times in Figure~\ref{endranks_cmp}.
% XXX: conclusion from these graphs?  Do we succeed?

\begin{figure}
\centering
\includegraphics[scale=.25]{native_endranks.png}
\caption{Similar to Figure~\ref{native_startrank}, this graph shows
the mean ending ranks and the standard deviation. As with start times,
end times vary sufficiently to make them poor predictors of interest.
\label{native_endrank}}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale=.25]{native_nonnative_endranks.png}
\caption{The mean end ranks for native interest compare to mean
end ranks for non-native interest. As before, there is a noticeable shift
downwards, but, as before, the means for the native interests tend to 
lie within the standard deviations of the non-native interests.
\label{endranks_cmp}}
\end{figure}

\paragraph{Download Rates Over Time.} Our final evaluation of anonymity examines
the rate of piece transmissions for native and non-native populations in the BitTorrent
Anonymity Marketplace. In other words, we verify that transmission \textit{patterns}
are indistinguishable.

We compute the number of requests for each node for a given torrent in time slices.  % XXX "per time slice?"  Ambiguous grammar.
All torrents are normalized to start at time slice 0. We then calculate all of the pieces
downloaded in subsequent time slices for native and non-native torrents. These amounts
are averaged and the standard deviation computed for each time slice. The resulting graph 
is a representation of the download pattern over time.

We created a composite graph plotting the download rates for all nodes across the entire simulation
in Figure~\ref{id1_composite_traffic}. This graph is the average of all the nodes' averages and
standard deviations for all torrents. As before, the native interests are downloaded
faster, but the download pattern for native torrents is within the standard deviation of the download
pattern for non-native torrents.
% XXX vocabulary alert: here it's "native interest".  Elsewhere we're using different terminology.
% Pick one thing, make a global pass, and get this straight.

Given that our primary goal was to obfuscate intent for any single neighbor, we also 
plotted the average of what each individual node sees from its peers in Figure~\ref{id1_clientview}.
% XXX average of what?
This graph was created by recording the pieces downloaded from individual nodes from its peers.
In other words, this graph represents the download patterns that a single node observers
during the lifetime of the simulation. These graphs demonstrate that we achieved our 
goals for indistinguishability.
% XXX the above text does nothing to explain to me what the graph shows.  I have no clue.

\begin{figure}
\centering
\includegraphics[scale=.30]{id1_composite_traffic.png}
\caption{Native and non-native traffic patterns super-imposed. While native traffic is above non-native traffic for the
same node, the median for the native is within the standard deviation of the 
other.\label{id1_composite_traffic}}
\end{figure}

\begin{figure}
\centering
\includegraphics[scale=.30]{native_nonnative_clientview.png}
\caption{This figure is similar to Figure~\ref{id1_composite_traffic} but limited to
the viewpoint of single clients. In other words, the former figure is a global representation
of download patterns, while this figure is representative of what a single peer observes.
\label{id1_clientview}}
\end{figure}

In view of these results, we revisit anonymity against each of the inquisitors that we previously identified.

% XXX: nuke the below three paragraphs?  We've already talked about these things before, right?
% (Or, maybe it's better to delete earlier mentions and bring these here.  
\paragraph{Passive Inquisitor.} These nodes do not directly interact with any actual 
nodes but only talk to the Tracker or, in our case, the DHT. The passive inquisitor can,
at best, track a given node's active set. From this information, it cannot determine the
node's native interest. As we demonstrated, the entrance and
exits of a given torrent in a node's active set behaves similarly regardless of the torrent's
status as native interest.

\paragraph{Decoy Passive Inquisitor.} These nodes directly interact with other nodes,
but do not actually exchange pieces. They can, however, advertise pieces and unchoke
other nodes. Such inquisitors gain additional information, but it is very 
little because rational nodes will drop them regularly for their poor performance.
However, with a Sybil attack~\cite{sybil}, these nodes can connect to a given node over and over
from different ip addresses, to simulate a continuous connection. Such a sybil node
could track the traffic of a rational node by listening to \texttt{Have} (piece) announcements.
Nevertheless, even a sybil node will not determine the node's native interest from this information
because, as we demonstrated, the download rates for a given
torrent for a node are similar regardless of the torrent's status as native interest.

\paragraph{Active Inquisitor.} The most powerful non-wiretap node, these nodes actively trade
with peers in the network. This feature allows them to attempt to ``trick'' a victim node
into revealing state by crafted trading. For example, an active inquisitor might obtain a large
number of blocks from all the nodes in active set. Then, it might selectively advertise these
blocks to the victim to see which blocks the victim takes a higher interest in. Furthermore, a very
well provisioned inquisitor might introduce \textit{identifiable torrents} into the marketplace that
it can use to manipulate torrent values within a neighborhood. The active inquisitor can use
such value manipulation to attempt to pierce the cloak of indistinguishability.

At present, we have not yet attempted to evaluate active inquisitors directly. Nevertheless, we expect
that unless the inquisitor can control a large portion of a victim node's local neighborhood (e.g.,
using a sybil attack, for example), it cannot have high confidence about the motivation for a node's
interest in any given torrent. This attack, however, is made not trivial because DHTs or trackers give out
random subsets of the peers to a participating node dramatically increasing the costs of overtaking a node's
neighborhood. Nevertheless, sybil is a significant
security issue and remains a point of research.

\subsection{Performance}

We chose to measure performance in terms of \textit{cost-to-acquire} and \textit{cost-to-complete},
as discussed previously. Again, these values are measured as multiples of the download 
size of the native interest.
% XXX: nuke earlier discussion, centralize it here.  No "as discussed previously".

The swarm, as a whole, behaved as we expected. The cost-to-complete averaged $5.71$ with
% XXX: what did you expect?  
a standard deviation of $0.43$. This value is very close to the optimal value of $k=5$ for these
tests. The costs-to-acquire were equally reasonable at an average of $3.12$ with a standard
deviation of $1.47$. 
% XXX: place standard deviations for both numbers alongside them, e.g., 3.12 +/- 1.47

What we did not see in our results was lower costs-to-acquire for more popular torrents. We are 
not entirely sure why this is so. It is possible that our simulations are just too small, with too
few torrents, or not enough real-world churn to observe this expected behavior. 
% XXX: and the final reviewer just decided to reject your paper.  Isn't this a good result?
% If the costs vary, wouldn't that compromise anonymity?  If you needed bigger simulations,
% why didn't you run them?

Further evidence of the limitations of our simulations are that we observed very little transitive 
trade. Transitive trading only accounted for less than one percent of all the piece exchanges. This
is because the relatively small marketplace we simulated allowed most of the participants to
find significant numbers of peers with whom they could trade directly. Nevertheless, it is 
positive that even in such a small world, peers were still able to make use of transitive trading.
% XXX: if it's used that infrequently, that means it's pretty much useless and it would be a bad
% idea to implement in a real system.  You should compare this to Scrivener, where transitive
% trading worked wonders.  But then Scrivener wasn't trying to achieve any sort of anonymity.

\subsection{Incentives}

In general, the BitTorrent Anonymity Marketplace provides strong incentives for cooperation,
because peers needing to maintain their anonymity have a natural incentive to carry
peer's interests for their own cover traffic. The ability to trade blocks transitively makes
them valuable in their own right.
% XXX: did you run any simulations to verify this?  Did you show that anti-social behavior
% wasn't rewarded?

But to evaluate our incentives in greater detail, we investigate them along two of three axes suggested by previous
work~\ref{faithfulness-formal, faithfulness-applied}.
% XXX: \ref or \cite?
In particular, we examine incentives for communication, and incentives for computation.
There is no need to evaluate incentives for message passing because the marketplace, like
regular BitTorrent, does not have peers relay messages for one another.

\paragraph{Incentives for Communication.} The first question is, \textit{does a rational node
have any incentive to lie about its state?} 
\begin{enumerate}
  \item \textbf{Active Torrents}: The only incentive for a node to lie about its active set is for
  increased anonymity against passive inquisitors. However, we have demonstrated that
  the native interest of a node is not revealed by the makeup and dynamics of the active set.
  Furthermore, the active set is necessary for performance and anonymity. Therefore, there
  is no incentive to lie about this state.
  \item \textbf{Choke Status}: There is no incentive for a rational node to misinform a neighbor
  about the choke state between them.
  \item \textbf{Piece-Interest Status}: The incentives of this part of inter-node communication
  is not clear. There is an incentive for a node to announce \texttt{Have} (piece) messages
  even for pieces it does not have because the value of the torrent in the marketplace will increase.
  On the other hand, unchoked neighbors may ask for these pieces and subsequently snub
  the lying node when it cannot produce them. We have not yet quantified these incentives.
  \item \textbf{Piece Requests}: A node does have an
  incentive to request pieces that it already has in order to drive the value of the torrent higher.
  However, it also affects the value of torrents by pretending not to have the piece.
  We have not yet quantified these incentives.
\end{enumerate}

\paragraph{Incentives for Computation.} The next question is, \textit{does a rational node
have any incentive to compute a non-conforming value for torrents in the marketplace?}
The answer is no by definition because nodes can choose their own market valuations. More
theoretically, all nodes have an incentive to develop effective methods of evaluating torrents
of non-native interest. The cooperation model supports and encourages this from of 
self-interested operation.

In summary, the Marketplace is built on a sound foundation of incentives, although some 
small components are currently manipulatable. These need to be improved in the
future.


==> objectives.tex <==
In this section, we clearly identify our objectives for the BitTorrent Anonymity Marketplace
as well as explicitly identify non-objectives.

\paragraph{Objective \#1: \textit{$k$-Traffic Anonymity}.} We assume a
threat model where an adversary can participate in torrent trading and
learn about any other node's full trading behavior. Despite this, we
wish nodes to preserve a degree of anonymity we call
$k$-\textit{traffic anonymity}, meaning that, in the worst case, the
strongest adversary can only conclude that a user was interested one
of $k$ different torrents, but cannot conclude which torrent was the
``true'' torrent of interest.

\paragraph{Objective \#2: \textit{Natural Incentives}.} A fundamental
goal in our system is that nodes should have natural incentives to
follow our protocol correctly. We wish to avoid the imposition of a
trusted third party which audits the network or the imposition of a
micropayment scheme. Just as BitTorrent rewards nodes who participate
faithfully in its tit-for-tat exchange protocol with a higher quality
of service, we wish to maintain this concept, despite the imposition
of anonymity mechanisms.

\paragraph{Objective \#3: \textit{Minimum Cover-Traffic Costs}.}
The pursuit of anonymity will come at a bandwidth cost.
We wish to ensure that for a given value of $k$-traffic anonymity,
the bandwidth overhead will be at most a factor of $k$, relative
to the cost of participating in any particular torrent. When we 
describe our design in detail, the significance of this issue
will become more apparent. 

In meeting these objectives, it is critical that we identify the objectives of different types of participants in the swarm.
%
\textit{Rational nodes} wish to achieve a given level of $k$-traffic
anonymity while maximizing download performance while and minimizing
upload contributions to other nodes.
%
\textit{Altruistic nodes} operate as seeds and expect neither
anonymity nor to download any particular object.
%
\textit{Inquisitors} participate in the system only to the extent that
they can identify which nodes are participating in which swarms, and
if possible to differentiate a node's natively desired torrent from any others. We
avoid the term \textit{attacker} because our system must be robust
against both attempts to violate anonymity and against
rational attacks~\cite{Nielson05Taxonomy}. Inquisitors are only
interested in the former and will not engage in the latter.
Ironically, the system must not only protect rational nodes from
having their intentions discerned by inquisitors, but must also
protect them from each other, as they themselves are the possible
\textit{rational attackers}.
% \textit{An inquisitor node's sole
% objective is to differentiate another node's download target from
% its cover-traffic.}

We can define different levels of strength for inquisitor nodes, with
stronger nodes having a greater ability to compromise anonymity.
%
\textit{Full passive} nodes do not participate in any tit-for-tat trading within a torrent.
They only scan BitTorrent trackers (centralized or distributed) for lists of participating nodes.
%
\textit{Decoy passive} nodes participate in the system, registering themselves as a 
participant, and responding to requests. However, they do not actually upload or download blocks although
they may announce otherwise.
%
\textit{Active} nodes participate and behave exactly as normal rational nodes will in all outward operations.

% XXX
%
% so here's a problem that's bugging me.  At this point, you've already got enough setup that you're ready to
% introduce your big ideas.  If you keep reading, even all the way through the "protocol design" section, you
% never lay out a short, clear, explanation of your design.  That really goes here, with your "protocol design"
% section really being more about fleshing out the details of your design.  Right now, you need to hit the
% high points:
%
% - we want nodes to participate in k different swarms, for a given level of k-anonymity
% 
% - we expect nodes to completely finish downloading the content in each of those swarms (otherwise
%    an inquisitor would be able to distinguish that they left early)
%
% - rather than having the user just pick all k swarms, which wouldn't offer the user any sort of defense
%    against a claim that they truly wanted any given torrent, we instead wish to have a design where
%    nodes look around, sort out what their neighbors are looking for, and offer to help them.  By doing
%    this, along with a notion of cross-swarm incentives (i.e., if you're good to me in one swarm and I
%    then see you later in another swarm, I'll return the favor), we can increase swarm sizes all around.
%
% At this point, you could skip directly to the hypotheses that you want to evaluate, then you're ready
% to get into your actual design.  This means that the non-objectives and assumptions below get
% shoved out.  Maybe they go later.
%
% I think I'm seeing this \section having three subsections
% - The opening (everything from the top to the beginning of this comment), which doesn't actually need a \subsection tag
% - our design sketch (this comment) plus the hypotheses (from below)
% - the assumptions and non-objectives
%
% Have a go at such a reorganization and see if it works for you.  If you don't like this, then at least
% hang onto the top-level goal, which is that you need to introduce your actual solution at some point
% in a coherent way.  The current text kind of leaks out the design, bit by bit, without ever forcefully
% presenting the ideas all in one place.

\paragraph{Architecture} We have designed the \textbf{BitTorrent Anonymity Marketplace} to achieve these objectives. We detail 
the protocol of the system in the next section, but there are three main concepts that drive the design.

\begin{enumerate}
\item Each node simultaneously participates in $k$ different torrents for $k$ anonymity. The composition of
these $k$ torrents can change over time.
\item Each node completely downloads at least $k$ different torrents for $k$ anonymity.
\item Each node chooses torrents for its $k-1$ cover traffic torrents that it believes will
help it acquire the torrent it actually wants. The BitTorrent Anonymity Marketplace allows
cross-trading so that a node can trade blocks in one torrent for another. The details of how nodes
value and trade torrents is detailed in the next section.
\end{enumerate}

It is worth discussing this design in terms of hypotheses as well as some assumptions 
that they are built upon. In future research,
some of these assumptions might become independent hypotheses for validation, but in the
context of this work, we accept them axiomatically.

\paragraph{Assumption \#1: \textit{Peers have a natural incentive to trade in blocks of cover traffic
if they believe that those blocks can help them acquire blocks of their true target.}} If we
assume that peers already expect to trade in some form of cover traffic, then it is reasonable to assume
that they have a natural incentive to pick cover traffic that is \textit{also} beneficial in some other
way. In other words, given a choice between neutral cover traffic, and cover traffic that has some
additional value, there is a natural incentive for a node to choose the latter.

\paragraph{Assumption \#2: \textit{Blocks from a given cover traffic torrent can be valuable to a node
if one or more peers is trading both that torrent and the node's true target.}} A node that wishes to
download some torrent needs to be unchoked by another node that can serve blocks from that
torrent. As stated previously, for a node to be unchoked, it must be one of the unchoking
peer's top uploaders. If uploading blocks of cover traffic to the peer gets the
node unchoked so that it can request blocks from its true target, then transmitting that cover traffic is
valuable to the peer.

\paragraph{Assumption \#3: \textit{Blocks from a given cover traffic torrent can be valuable to a node
if one or more peers is trading both that torrent and another torrent that the node views as valuable.}}
A torrent's value can be transitive. Once a node affixes some kind of
value to a acquiring any given torrent, then trading any other torrent that can help the node acquire its true target is
also valuable. The process is recursive. Torrent blocks that
can be traded for the true target's blocks are more valuable than torrent blocks that must be traded for
other torrent blocks that can finally be traded for the true target's blocks.
% the above section was written in a confusing way.  I tried to clean it up. - dwallach

\paragraph{Assumption \#4: \textit{Blocks from cover traffic torrents are more valuable to a node
depending on the supply of and the demand for those blocks in the node's neighborhood.}}
When a node selecting a cover-traffic torrent, it will place higher value on torrents
that provide the most leverage in acquiring higher-valued torrents. Within the node's neighborhood,
more neighbors desiring a given torrent constitutes
\textit{demand} for that torrent. At the same time, more peers in the neighborhood providing blocks
constitute a \textit{supply}. The higher the demand and the lower the supply,
the more valuable the torrent.

\paragraph{Assumption \#5: \textit{The supply and demand of a given torrent can be estimated
from a node's interactions with its peers.}}
While any given BitTorrent node cannot gain a global view of torrent popularity, it can observe
what is being advertised and traded within its neighborhood. Neighborhoods are large enough
to provide a useful sample of popular behavior everywhere else.
% Unfortunately, a node cannot fully determine the supply
% and demand for a given torrent. For example, the number of requests that a neighbor has out
% for a torrent should affect the node's calculation of demand, but this information is not available.
% However, the state information available is enough to produce a sufficient estimate.

\paragraph{Hypothesis \#1: \textit{None of the identified classes of inquisitor can distinguish a 
node's interest in a torrent as true interest or simply the result of supply and demand influences
in a node's local neighborhood.}} A non-colluding inquisitor observing BitTorrent state information
revealed by another node will be unable to determine if interest in a given torrent is because the
node actually wants it, or if it is simply requesting it because a high valuation driven by
local supply and demand conditions. It should be noted that a non-colluding inquisitor cannot
determine a node's local neighborhood except in degenerate swarms where the swarm
size is smaller than neighborhood size.
% XXX the italics sentence and the one after it say basically the same thing.  Please condense.

\paragraph{Hypothesis \#2: \textit{With correct parameterization for supply and demand calculations,
participation in the marketplace will converge with predictable download costs.}} The value of a torrent
to a node is going to depend on a number of factors and can change as the neighborhood changes.
However, with effective parameterization of the torrent-value calculation, a marketplace swarm
can have a strong probability of completing $k$ downloads with predictable total costs.

\paragraph{Hyptohesis \#3: \textit{The marketplace can be designed such that participating self-interested nodes
remain faithful to the specified design.}} In other words, we believe that our design can provide
effective incentives for obedience of rational nodes to the designed protocol.
% XXX do you meant to use the term 'strategy-proof' here somewhere?

As an important side note, we emphasize that our design provides no additional anonymity guarantees.
A few are worth disavowing explicitly.


\begin{itemize}
\item \textbf{Identity Masking}. Unlike Tor, neither identity nor location are concealed in any way. 
\item \textbf{Effective cover traffic}. The Marketplace makes no guarantee about the nature of its
cover traffic. It is conceivable that every torrent that a node is downloading could be equally
``embarrassing.''
\item \textbf{Collusion Resistance}. Colluding neighbors could combine information to analyze 
a peer's behavior. If all of the neighbors of a peer collude, all $k$-traffic-anonymity is lost. 
How many peers are required to collude to identify a peer's native interest is a subject of future
research.
\item \textbf{Line Tap Resistance}. Our design obscures a peer's intent from its neighbors. Much as if
all of a peer's neighbors are colluding, a wire-tap or packet sniffer would expose a peer's entire
communication stream and expose intent. In Section~\ref{discussion} we discuss how to harden the
system against most powerful adversaries. % such as organizations that can perform
%passive or active wire-taps.
\end{itemize}



==> protocol_design.tex <==
In this section we detail how Marketplace protocol deviates from BitTorrent
and the details of its algorithms.

\subsection{Definitions}
% XXX can we move all of this later?  Or move the definitions from up here to being in-line?
% We need to cut directly to the actual design.  We're already on page 6 and haven't said
% hardly a word about how our stuff works!
The BitTorrent Anonymity Marketplace requires a few additions to
the nomenclature:

\begin{itemize}
\item \textit{Native Interest}: A node's actual download target. For our purposes, 
there is only one. Everything else is cover traffic.
\item \textit{Active Set}: The $k$ torrents for which the node is currently trading. The Active
Set may change over time, and a node that enters the Active Set is not guaranteed to completely download.
\item \textit{Download Set}: The $k$ or more torrents that the node completely downloads. 
Every node in the Download Set will, at one time or another, been in the node's active set, but the
reverse is not true.
\item \textit{Cost-to-Acquire}: The amount of data that must be downloaded before the node has
a completed the download of its native interest. This value is expressed as a multiplier of the
size of the native interest.
\item \textit{Cost-to-Complete}: The amount of data that must be downloaded before the node
can exit the swarm. This value is expressed as a multiplier of the size of the native interest. It
will always be at least $k$.
\item \textit{Cross-trading Distance}. As stated in hypothesis 3, the value of any given torrent
to a node is based on eventually getting blocks from the node's native interest. This can be 
modeled as a tree where the root is the native interest and the children of each node are the
torrents that can be traded for their parent. The cross-trading distance is the distance from a
torrent to the native interest at the root.
\item \textit{Sensitivity}. The subjective value we use to describe how a node perceives the risk
of downloading. A torrent may be sensitive to a node for legal, political, or personal reasons.
\end{itemize}

\subsection{High-level Design}

\paragraph{DHT.}  For convenience purposes we have chosen to maintain state 
about the Marketplace in the form of a Distributed Hash Table
(DHT), but our results could apply to a modified tracker as well. The DHT provides nodes with active torrents
and the peers currently trading those torrents.  In the
simulation, the DHT is idealized as a global dictionary. In a real implementation,
DHT security is an issue but outside the scope of this paper and already discussed in other work~\cite{something}.

\paragraph{Publishing.} It is essential that objects exchanged in the Marketplace are 
opaque to users that are uninterested in them. Otherwise, users may
choose to not trade in objects they deem overly sensitive. For this
reason, all content is encrypted and identifiers are random.
% XXX this is an important point!  This is high level design!  This is
% the stuff you want to lead with, not the DHT business.
Publishers must provide a means for obtaining the random identifier
that maps to the published content through some out-of-band
method. The forward mapping would be trivial, but the reverse mapping
would be difficult to discover. In this manner, participating nodes will
trade in many torrents without any knowledge of their content, except
for their own native interest.

Once the publisher has encrypted the object, and created the random
id, it generates a torrent-file-like record. This record stores the random
identifier, the hash of each piece of the encrypted file, the number of
pieces and so forth. The publisher then inserts this record into the
DHT and joins one or more nodes to the DHT as seeds for the
object. Obviously, this is not compatible with current BitTorrent clients
but is achievable with minimal modifications.

\paragraph{Messages.} All inter-peer communication consists of unmodified 
BitTorrent messages with one exception. While normal BitTorrent messages 
include the appropriate torrent identifier, the \texttt{Choke} and \texttt{Unchoke}
messages in the Marketplace are not torrent-specific. These two messages
signal that the sender is willing or unwilling to fulfill requests
for any of the torrents it is currently advertising. For this reason, instead of
including a torrent identifier, these two messages
use an identifier for the DHT. All other messages in the Marketplace 
remain unchanged from stock BitTorrent.

\paragraph{Joining.} To use the BitTorrent Anonymity Marketplace, a participant first
acquires the random identifier for the desired object from an out-of-band
channel provided by the publisher. Next, the node joins the
DHT and requests a list of active torrents. From this list the node creates
a list of $k$ torrents consisting of its desired torrent plus $k-1$ random torrents
from the list. The node then indicates to the DHT that it is joining those
K torrents and requests participating peers.

With these peer lists, the newly joining node begins constructing its
neighborhood. Initially, it evenly splits its total peer connections among each
of the $k$ torrents. Each node connects with other peers on a per-torrent basis.
As peers can, and should, overlap in multiple swarms, two peers may share
multiple connections. Additionally, peers exchange messages about all the
torrents in their active set, not just the ones that they have in common.

Each node connects
to another peer using the standard BitTorrent approach of using
a TCP connection. It uses one connection for each torrent in its
active set. As the other peer will also respond with connections for
each torrent, the two peers could potentially have $2\times K$
connections initially. However, after an initial exchange of metadata,
the un-shared connections are dropped.

\paragraph{Trading.}  After nodes join the system, they unchoke peers in a manner similar to BitTorrent
with the highest upload services getting the unchoke slots. However, in the Marketplace,
all upload service is adjusted by the value the receiver places on the pieces being
uploaded. Our current design keeps the value constant across an entire torrent
for performance reasons, but could be extended to be per-piece.

As with stock-BitTorrent, unchoking is handled every 30 seconds based on the
top three or four uploading neighbors plus one or two optimistic unchokes. However, 
in selecting the the top uploaders, the node first re-computes the value of each torrent in its
active set and adjusts the value of a neighbor's upload contribution by the value of the torrents
it uploaded.

In addition to managing the chokes and unchokes the node also adjusts its set of $k$
active torrents. The node drops its least valuable torrent if a more valuable
torrent has become available at regular intervals. 

\paragraph{Seeding and Termination.} A Marketplace participant must complete $k$ downloads before leaving the system. Any
torrent not completely downloaded will not serve as effective cover traffic. As we noted previously,
a node may trade in a torrent and then drop it because it is not significantly valuable. In short,
the total number of torrents that may have ever been in a node's active set might be considerably higher
than $k$, but the size of the download set must always be at least $k$.

When a torrent is completed, be it the native interest or not, the node continues to participate
normally in the Marketplace. In this form, the node is not technically seeding. Although the
torrent has been downloaded, and the node may still serve blocks from it, it is doing so on
exchange for blocks from other torrents.

Nodes can choose to enter a seed-only phase where they only upload. They can seed
any number of torrents they wish.

\subsection{Marketplace Algorithms}

\paragraph{Computing Torrent Value.} The value that each node places on a given non-native interest
torrent is essential to all other operations. It is used to derive the number 
of peers to contact for each torrent, the value of uploads particular blocks to particular neighbors, and 
the composition of the active set of torrents being traded.

The primary consideration in computing this torrent value is how much leverage it will provide the node
in acquiring its native interest. We assume that the economic principles of supply and demand apply to
our Marketplace and, therefore, demand divided by supply provide a reasonable accurate indication of
how much leverage a torrent provides. For example, if many nodes are interested in downloading some
torrent, but few nodes in the neighborhood have pieces of the same, then that torrent is highly valuable.

Unfortunately, the BitTorrent protocol  

If BitTorrent provided a mechanism for accurately
measuring these two factors, the formula would be simple.

Our algorithm for evaluating a torrent was developed experimentally.
% XXX (redundant text commented out)
% The fundamental
% principle was, from the beginning, to compute supply and demand of a torrent
% for a node in a neighborhood. But the full state of the neighborhood is not available
% to a node forcing it to compute a supply and demand estimate. 
In the course of this research, we identified several factors that improved
our system's performance:

% XXX: aaiiigggh, more lists of stuff, but this time it's actually necessary.
\begin{enumerate}
\item \textit{Cross-trading Distance}. As described previously.
\item \textit{Approximate Supply}. We approximate the supply of a torrent by how
many pieces of the torrent are available across all nodes in the local neighborhood.
\item \textit{Approximate Demand}. As an analog to the previous factor, the base demand is
calculated from the total number of pieces of the torrent that would be required to
satisfy all the nodes in the local neighborhood. This is a very rough approximation because
the node has very little information to help it determine if its peers are actively interested
in the torrent. The remaining factors help the node improve its own valuation of 
a torrent and/or its guesses about other nodes valuations.
\item \textit{Activity}. Sometimes, a node can receive hints about its peers current interests.
When peers receive a full piece, they announce it to the neighborhood with a \texttt{Have}
message. From such messages, a node can determine which torrent a peer is actively
trading, and adjust its estimation of demand accordingly.
\item \textit{Direct Requests}. If the node receives direct request messages, it can be completely
sure that the peer making those requests has a high interest in the torrent and adjusts its
estimation of demand accordingly.
\item \textit{Completion}. Nodes wish for complete downloads. Anonymity is 
not preserved without downloading $k$ torrents. To achieve convergence in
downloading, as a node nears completion, its value increases.
\end{enumerate}

Using these factors, we compute the value for each torrent as follows:

\begin{enumerate}
\item Let the torrent's cross-trading distance be $d_{cx}$
\item Let the number of peers in the local neighborhood be $N$
\item Let the number of peers that trade in this torrent be $M$
\item Let the base multiplier $b = \frac{1}{2^{d_{cx}}} \times \frac{M}{N}$
\item Let supply $s$ be the number of pieces of this torrent available in the local neighborhood
\item Let demand $d$ be the number of pieces of this torrent missing in the local neighborhood
\item Let demand-multiplier $R$ be the number of request messages for this torrent since the last update.
\item Let activity $a$ be the number of have messages for this torrent since the last update.
\item Let $F$ be the size of the object in bytes.
\item Let $L$ be the bytes left to download.
\item Compute the completion multiplier as $c = MIN(1, \frac{F}{L})$
\item Compute the value of torrent $A$ as $V(A) = b(\frac{d}{s} + a + R + c)$
\end{enumerate}

The purpose of the base multiplier $b$ is to reflect that the value of a non-native interest
torrent is in its capacity to leverage trades for native interest blocks. The further the cross-trade
distance, the less valuable the torrent. 
% XXX and this is where your paper gets summarily rejected.  A reviewer reads this and says
% where did all these equations come from?  This seems completely ad-hoc.  Where are the
% principles that led to these equations?  Has anybody else done anything else like this in the past?

Supply and demand is used as the basic measure of how valuable a torrent is. Activity $a$ is
used to determine how active the trading of a particular torrent's blocks are. In monetary terms,
activity might be how ``liquid'' the blocks of a particular torrent are. Demand multiplier $R$ 
indicates that we are receiving actual requests for this torrent, making them more immediately
valuable. Finally, the completion multiplier values more complete downloads higher. This improves
stability so that downloads in progress are less likely to get kicked out of the Active Set because
of a ``faddish'' upstart torrent.

To determine that these values actually matter to the marketplace, each was affixed was multiplied
by a coefficient. Adjusting the coefficient of one value while holding the other values fixed allowed
us to experimentally evaluate its importance. Each parameter, when negated with a zero-coefficient
had a negative impact on performance, and would often prevent the system from converging. For
the final simulations used in the evaluation section, we picked the coefficient for the parameter
that produced the best performance. 

Please note that we do not claim that this algorithm is optimal, nor that the 
coefficients chosen are optimal under all, or any, circumstances. In the real world, clients could
chose to use parameters of their choosing. From a game-theoretic viewpoint, the system benefits
when nodes successfully use cover-traffic to leverage their native-interest. Therefore, there
is no risk to system stability from nodes modifying their evaluation calculations.
% XXX this paragraph further drives the knife in for reviewers who were previously on the fence.
% I've complained about this before.  Your techniques are completely ad-hoc.  Where's the
% economic theory or game theory or whatever to backstop what you've done?

\paragraph{Determining Peer Composition.} When adding peers to the neighborhood, a node
must decide which torrent from its active set it wishes to draw them from. Our algorithm is to
draw nodes from a torrent proportional to the value of that torrent. When the node first joins
the Marketplace, all torrents values are zero, so every torrent contributes an equal number of
peers.

\paragraph{Updating the Active Set.} At a specified interval, the node drops its least valuable torrent
for a more valuable one if one exists. 
The node knows about other torrents from its neighborhood
as the peers therein signal the torrents they are participating in, even if they are not shared. A node
can compute values for non-active torrents but without have or request messages, the activity multiplier
is always just $\frac{1}{t}$. This means that active torrents are always more valuable than non-active
torrents, but if an active torrent has stalled, another torrent has the capacity to take its place.
We picked a fifteen minute interval based on experimental testing.

Significantly, a node's native interest can drop out of the active set. This is important because it means
that an observer cannot be absolutely certain that a node's current active set contains its native 
interest. Although we have described our system as having a node always choose the native interest
as one of the initial members of the active set, a node that wishes to improve its anonymity can choose
an entirely random initial active set at initialization and wait for the native interest to cycle into activity.

To facilitate finding better torrents and cycling the native interest back into activity, when updating the
active set, the node can choose to occasionally chose a random torrent to cycle into activity. This is
analogous to an optimistic unchoke. In value terms, it can be seen as an investment. Even if the node
detects no significant activity in the selected torrent, \textit{its} activity in the torrent may increase
its value and draw other nodes into participation\footnote{Incidentally, this behavior is sometimes
seen in real-world stock markets and is called a \textit{self-fulfilling prophecy}.}.
% XXX: on the other hand, this stuff is much more interesting.

% XXX: broad recommendation: ditch all the math for the algorithm in this section.  Cut it all.
% Instead, talk about how you assign coefficients to a list of different things (and list them),
% and your design/implementation/review process took many spins around the block looking
% for algorithms that performed well on your rough metrics.  

% I'll point out that you never use any of these equations later in the paper.  That's all the more
% reason to eliminate them here and be more handwavy.  At least you end up drawing less
% attention to your ad-hoc design process.

